Why Capsule Neural Networks Do Not Scale: Challenging the Dynamic Parse-Tree Assumption

Capsule neural networks replace simple, scalar-valued neurons with vector-valued capsules. They are motivated by the pattern recognition system in the human brain, where complex objects are decomposed into a hierarchy of simpler object parts. Such a hierarchy is referred to as a parse-tree. Conceptually, capsule neural networks have been defined to realize such parse-trees. The capsule neural network (CapsNet), by Sabour, Frosst, and Hinton, is the first actual implementation of the conceptual idea of capsule neural networks. CapsNets achieved state-of-the-art performance on simple image recognition tasks with fewer parameters and greater robustness to affine transformations than comparable approaches. This sparked extensive follow-up research. However, despite major efforts, no work was able to scale the CapsNet architecture to more reasonable-sized datasets. Here, we provide a reason for this failure and argue that it is most likely not possible to scale CapsNets beyond toy examples. In particular, we show that the concept of a parse-tree, the main idea behind capsule neuronal networks, is not present in CapsNets. We also show theoretically and experimentally that CapsNets suffer from a vanishing gradient problem that results in the starvation of many capsules during training.

==> capsnet_parse_tree.tex <==
%TODO  THE PARSE TREE IS DEFINED BY THE CapsNet.
%TODO Maybe add one more sentece to how this creates a tree like structure
%TODO Maybe elaborate on the role of routing

\subsubsection*{How the CapsNet defines a parse-tree}
In general, a tree is a discrete data structure and might be generated by dynamically allocating memory, depending on the number and types of nodes and edges required ~\cite{icann/HintonKW11}~\cite{nips/SabourFH17}.
However, this is not effectively realizable with current deep learning approaches that operate in the continuous space and rely on fixed-sized parameter and input dimensions.

%
% Fuzzy Parse-Tree
%
Instead, the CapsNet implements a fuzzy tree with capsules representing fuzzy nodes and coupling coefficients representing fuzzy edges.

The CapsNet calculates a fixed number of hierarchically ordered capsules, where each capsule $U_{(i,:)}^l$ in layer $l$ is connected to each capsule $U_{(j,:)}^{l+1}$ in layer $l+1$ via a coupling coefficient $C^l_{(ij)}$.

The squashing function~\eqref{eq:sqash} ensures that each capsule has its length in $[0, 1)$, which is interpreted as the capsule's probability of being present in the parse-tree.

The routing algorithm Alg.~\ref{alg:capsnet_routing} calculates the coupling coefficient matrix $C^l$.
The row-wise softmax ensures that the votes $\hat{U}^l_{(i,:,:)}$ of a lower layer capsule $U^l_{(i,:)}$ are multiplied with weights $C^l_{(i,:)}$ that sum up to one.
We can view the coupling coefficients as fuzzy edges with $U^l_{(i,:)}$ being connected to $U^{l+1}_{(j,:)}$ with probability $C^l_{(i,j)}$.

The multi-layer hierarchy of squashed capsule nodes, connected by its coupling coefficient edges, defines a fuzzy tree.
%
% How should this semantically work?
%
\subsubsection*{CapsNet connection to the capsules idea}
In~\cite{nips/SabourFH17}, it is hypothesized that the network learns to associate a capsule with a dedicated visual entity within the input images and represents the entity's probability of presence with the capsule's magnitude and the entity's instantiation parameters with the capsules direction.

Slightly changing the viewpoint on an entity does not affect its presence within the scene but only its instantiation parameters. The respective capsule's magnitude should be unaffected, whereas the capsule direction changes.

This behavior makes the parse-tree viewpoint invariant and the capsules direction viewpoint equivariant.
Subsequently, the CapsNet, at least in theory, should exhibit outstanding robustness to affine transformations of the input data and generalize well to novel viewpoints.

Furthermore, as the votes of capsules in lower layers collectively determine the activation of a higher layer capsule, depending on the similarity of their votes, it was hoped that the hierarchically connected capsules represent visual entities that stand in part-whole relationship to each other.

\ignore{
\begin{figure*}[th]%
	\centering
	\subfloat[
	A tree (left) can be represented by multiple layers of capsules (right).
	Active capsules ($\norm{u_i^l} \approx 1$) in consecutive layers are connected by strong coupling coefficients $c_{ij} = 1$.
	The coupling coefficients from and to inactive capsules  ($\norm{u_i^l} \approx 0$) is not shown.
	]
	{\includegraphics[width=0.46\textwidth]{figs/imgs/parse_tree_capsules.png}
		\label{fig:misc:capsnet:fuzzy_parse_tree}}%
	\qquad
	\subfloat[
	Creating a two-level tree from capsules. The nodes a re capsules with their length representing their probability of being persent in the parse-tree. The coupling coefficient denote the probability of an edge being present.
	]
	{\includegraphics[width=0.46\textwidth]{figs/imgs/capsules_parse_tree.png}
		\label{fig:misc:capsnet:fuzzy_parse_tree_values}}%
	\caption{The CapsNet fuzzy parse-tree}
	\label{fig:misc:capsnet:parse_tree}
\end{figure*}
}

==> capsnet_section.tex <==
%
% CAPSULES ARENT FORMALLY DEFINED NOT IS THE PARSE TREE. BUT CAPSNET DEFINE A PARSE TREE!
% DESCRIBE CAPSNET ABSTRACTLY
%
A generic capsule neural network (CapsNet) consists of a backbone function that maps images to feature matrices, $\ell$ routing layers, and a reconstruction network. In the follwing we introduce basic notations and definitions, the generic CapsNet architecture, and a loss function for training CapsNets. Furthermore, we discuss how CapsNets define a parse tree and the connection of CapsNets to the abstract idea of capsules. 

\subsubsection*{Architecture}
An illustration of the CapsNet model is shown in Fig.~\ref{fig:cn:architectures}.
A capsule is a vector $u \in \mathbb{R}^d$ with $\norm{u}_2 \in [0, 1)$.
The CapsNet calculates a multi-layer hierarchy of capsules with $U^l \in \mathbb{R}^{(n^l \times d^l)}$ holding $n^l$ capsules of dimension $d^l$ in layer $l$.

First a backbone function $\phi(\cdot)$ extracts feature maps $F\in \mathbb{R}^{(h\times w\times c)}$ from an input image $X^{(h_x\times w_x\times c_x)}$.
Those feature maps are reshaped into the form $S^0 \in \mathbb{R}^{(n^0 \times d^0)}$, holding a number of $n^0$ vectors of dimension $d^0$.

The first layer of capsules  $U^{0} \in \mathbb{R}^{(n^0\times d^{0})}$, also called PrimeCaps, is obtained by a non linear transformation $U_{(i,:)}^0 = g(S_{(i,:)}^0)$ with the squashing function  $g:\mathbb{R}^n \rightarrow \mathbb{R}^n$, that "squashes" the length of a capsule in the range $[0, 1)$. In this work, we use a slightly modified squash operation, that behaves similarly but is more sensitive to small changes near zero ~\cite{DBLP:corr/Xi2017}, which is required to stack multiple routing layers:
\begin{flalign}
g(s) = \left(1 -\frac{1}{\exp(\norm{s}_2)} \right) \frac{s}{\norm{s}_2} \label{eq:sqash}
\end{flalign}
%\begin{flalign}
%	g(s) = \frac{\lVert s \rVert^2}{1 + \lVert s \rVert^2} \frac{s}{\lVert s \rVert} \label{eq:sqash}
%\end{flalign}
From there, each consecutive layer of capsules $U^{l+1} \in \mathbb{R}^{(n^{l+1} \times d^{l+1})}$ is calculated from the previous layer of capsules $U^{l} \in \mathbb{R}^{n^l \times d^l}$.
For each lower layer capsule $U_{(i,:)}^l$ and for each upper layer capsule $U_{(j,:)}^{l+1}$, there is a linear transformation:.
\begin{flalign}
	\hat{U}_{(i,j,:)}^l = U_{(i,:)}^l W_{(i,j,:,:)}^l
\end{flalign}
With parameter tensor $W^l \in \mathbb{R}^{(n^l\times n^{l+1}\times d^l\times d^{l+1})}$ and $\hat{U}^l \in \mathbb{R}^{(n^l\times n^{l+1}\times d^{l+1})}$ being called votes.
An upper layer capsule $U_{(j,:)}^{l+1}$ is then the squashed, weighted sum over all votes of the lower layer capsules $\hat{U}^l_{(:,j,:)}$:
\begin{flalign}
	U_{(j,:)}^{l+1} = g\left(\sum_{i}C_{(i,j)}^l \hat{U}_{(i,j,:)}^l\right)
\end{flalign}
The weights $C_{(ij)}^l$ are called coupling coefficient with $\sum_{j} C^l_{(ij)} = 1$ for $i$ being fixed.
They are determined by an iterative routing algorithm, see Alg.~\ref{alg:capsnet_routing}.

\subsubsection{Training}
The CapsNet uses the Adam optimizer to learn the parameters within the backbone function $\phi(\cdot)$ as well as the weight Tensors $W^{l}$ in each layer by minimizing the $\alpha$-weighted sum of a supervised classification loss $L_m$ and an unsupervised reconstruction loss $L_r$:
\begin{flalign}
L = L_m + \alpha \cdot  L_r
\end{flalign}

The number of output capsules in the last layers $U^{-1}$ is set to match the number of $k$ classes in the respective dataset and the length of the $j$-th capsule $u_j^{-1}$ is interpreted as the probability of the $j$-th class being present in the input.

The margin function is applied to the last layer of capsules to compute a classification loss $L_m$:
\begin{flalign}
L_m =\sum_{k} T_k \max(0, m^+ - \norm{u_k^{-1}})^2 + \\ \lambda(1 - T_k)\max(0, \norm{u_k^{-1}} - m^-)^2
\end{flalign}
where $T_k$ is 1 if the object of the $k-th$ class is present in the input and $0$ otherwise.

Output capsules $U^{-1}$ that correspond to classes $k^{-1}$ that are not present in the input image $X$ are masked out by zeros. All the capsules are then concatenated and fed into a generator network $\psi(\cdot)$, that is tasked to reconstructs the input and the loss is the sum of squared distances between the reconstruction and the pixel intensities:
\begin{flalign}
L_r = \sum_{h,w,c}(X_{h,w,c} - \psi(mask(k^{-1}, U^{-1}))_{h,w,c})^2
\end{flalign}

During inference, the procedure changes slightly. There we mask out all but the capsule with the largest norm.

\begin{figure}
\begin{algorithm}[H]
	\caption{routing-by-agreement}\label{alg:capsnet_routing}
	\textbf{Input}: $\hat{U}$, $r$ \\
	\textbf{Returns}: $C$
	\begin{algorithmic}[1]
		\State $B_{(i,j)} \gets 0$
		\For{$r$ iterations}
		\State $C_{(i,j)} \gets \frac{\exp(B_{(i,j)})}{\sum_{k}\exp(B_{(i,k)})}$
		\State $S_{(j,:)} \gets \sum_{i}C_{(i,j)} \hat{U}_{(i,j,:)}$
		\State $V_{(j,:)} \gets g(S_{(j,:)})$
		\State $B_{(i,j)} \gets B_{(i,j)} + \sprod{\hat{U}_{(i,j,:)}}{V_{(j,:)}}$
		\EndFor
	\end{algorithmic}
\end{algorithm}
\caption{The routing algorithm calculates the coupling coefficients $C \in \mathbb{R}^{(n^l\times n^{l+1})}$ from the lower layer capsule votes $\hat{U} \in \mathbb{R}^{(n^l\times n^{l+1}\times d^{l+1})}$}
\end{figure}


\begin{figure*}[!ht]
	\centering
	\subfloat[
	CapsNet for the MNIST classification tasks, consisting of two convolutional layers that output the PrimeCaps. A single routing layer yields the DigitCaps. After masking the digit caps are fed into a reconstruction network.
	]
	{\includegraphics[height=0.172\textheight]{figs/imgs/capsnet_original.pdf}
	 \label{fig:cn:architecture_original}}%
	\qquad
	\subfloat[
	General Capsnet consisting of a backbone function yielding a first layer of capsules. Each consecutive layer of capsules is calculated via a routing algorithm.
	]
	{\includegraphics[height=0.172\textheight]{figs/imgs/capsnet_general.pdf} \label{fig:cn:architecture}}%

 \caption{The original MNIST CapsNet on the left and the general CapsNet model on the right.}
 \label{fig:cn:architectures}
\end{figure*}


==> complexity_analysis.tex <==
\section{Complexity Analysis} \label{app:complexity_routing}

Understanding as a mapping from vectors to vectors, we can compare it to Transformers.
$U^{l} \in \mathbb{R}^{n \times d} \rightarrow U^{l+1} \in \mathbb{R}^{n \times d} $

\textbf{Visual Transformer - Encoder Layer}

Multi-Head Self Attention~\cite{iclr/DosovitskiyB0WZ21}.
\begin{flalign}
	[Q, K, V] = U^l W_{QKV} \\
	A = \sigma (QK^T / \sqrt{D_h}) \\
	SA = AV \\
	MSA(U^l) = [SA_1, ..., SA_k] W_{msa}
\end{flalign}
Parameters
\begin{flalign}
	W_{QKV} (k \times 3 \times d \times d_h) \\
	W_{msa} (k \times d_h \times d)
\end{flalign}
with $d_h = d /k$
\begin{flalign}
	W_{QKV} (3 \times d \times d) \\
	W_{msa} (d \times d)
\end{flalign}
Memory: $4 \times (d \times d)$, $O(d^2)$ and controll its nu.\\
Time: $O(n^2 d + n d^2)$

\textbf{CapsNet - Routing Layer} \\

Calculation from mapping vectors in CapsNet routing layers $U^{\ell} \in \mathbb{R}^{n \times d} \rightarrow U^{l+1} \in \mathbb{R}^{n \times d} $. The routing algorithm considers learned parameters and also different intermediate results for each routing layer $\ell$ in the capsule model $L$. \\  

Parameters:
\begin{itemize}
	\item $W (n^l \times n^{\ell+1} \times d^{\ell}  \times d^{\ell+1}), O(n^\ell \times n^{\ell+1} \times d^{\ell}  \times d^{\ell+1})$
	\item  $B (n^\ell \times n^{\ell+1}), O(n^\ell \times n^{\ell+1})$
\end{itemize}

Intermediate results:
\begin{itemize}
	\item $\hat{U}^\ell (n^\ell \times n^{\ell+1} \times d^{\ell+1}), O(n^\ell \times n^{\ell+1} \times d^{\ell+1})$
	\item $S (n^{\ell+1} \times d^{\ell+1}), O(n^{\ell+1} \times d^{\ell+1})$
	\item $V (n^{\ell+1} \times d^{\ell+1}), O(n^{\ell+1} \times d^{\ell+1})$
	\item $C (n^\ell \times n^{\ell+1}), O(n^\ell \times n^{\ell+1})$
	\item $U (n^\ell \times d^{\ell}), O(n^\ell \times d^{\ell})$
\end{itemize}

The sum of parameters $n_p$ and intermediate results $n_i$ can be calculated with respect to the number of layers. 

\begin{flalign}
	n_p =\sum_{\ell=0}^{L} (n^\ell \times n^{\ell+1} \times d^{\ell} \times d^{\ell+1}) + (n^\ell \times n^{\ell+1})
\end{flalign}	

\begin{flalign}
	n_i =\sum_{\ell=0}^{L} (n^\ell \times n^{\ell+1} \times d^{\ell+1}) + 2 \cdot (n^{\ell+1} \times d^{\ell+1}) + (n^\ell \times n^{\ell+1}) +  (n^\ell \times d^{\ell})
\end{flalign}	

with $ (n^\ell = n^{\ell+1}, d^{\ell} = d^{\ell+1})$ \\
Memory: $O(\ell \times n^2 \times d^2)$ \\
Time: $O(\ell \times n^2 \times d^2)$ \\

==> investigation_model_performance.tex <==
Our findings stand in line with previous work~\cite{acml/PaikKK19}~\cite{cvpr/GuT20}~\cite{cvpr/GuT021}  and therefore we do not elaborate on these results. These findings include:
On AffNIST, the baseline models trained with uniform routing invariably outperform models trained with RBA. Uniform routing sets all the entries in the coupling coefficient matrix to a fixed value, disregarding the idea of agreement(Tab.~\ref{tab:affnist:grid_run:best_overall_models}). This observation indicates underlying issues concerning the routing algorithm.
In general, while a higher number of capsules positively affects the model's performance, both the dimension and depth correlate negatively with affine robustness and classification performance. (Tab.~\ref{tab:affnist:grid_run:best_models_depth}.).
On CIFAR10, depth severely worsens classification performance (Tab.~\ref{tab:cifar10:grid_run:best_models_depth}).
Furthermore, there seems to be an inherent limitation in depth, as depending on the exact parameter choice, we could not successfully train models deeper than 8-12 routing layers.

All these findings and previous work suggest a scaling issue underlying the dynamic routing algorithm.

==> notation.tex <==
We use the following notation and variable names. In general lower case Latin letters denote vectors and scalars, and upper case Latin letters denote matrices and higher dimensional tensors.  
\begin{itemize}
	\item $\phi: \mathbb{R}^{(h_x\times w_x\times c_x)} \rightarrow \mathbb{R}^{(h_f\times w_f\times c_f)}$ ... feature extracting backbone
	\item $\psi:\mathbb{R}^{(n \times d)} \rightarrow  \mathbb{R}^{(h_x\times w_x\times c_x)}$ ... reconstruction network
	\item $g:\mathbb{R}^d \rightarrow \mathbb{R}^d$ ... non linear squashing function
	\item $X \in \mathbb{R}^{(h_x\times w_x\times c_x)}$ ... input image tensor
	\item $F \in \mathbb{R}^{(h_f\times w_f\times c_f)}$ ... feature map tensor
	\item $s \in \mathbb{R}^d$ ... unnomalized capsule vector
	\item $S \in \mathbb{R}^{(n\times d)}$ ... matrix holding $n$ unnormalized capsules of dimension $d$.
	\item $u \in \mathbb{R}^d$ ... normalized  capsule vector $u = g(s)$
	\item $U \in \mathbb{R}^{(n \times d)}$ ... matrix holding $n$ capsules of dimension $d$
%	\item $u \in \mathbb{R}^d$ ... a capsule vector
\end{itemize}
We use subscripts in brackets for dimension dependent element selection and unless differently specified, the superscript $l$ on variables denotes the layer index.
\begin{itemize}
	\item $U_{(i,:)}^l \in \mathbb{R}^d$ ... $i$-th capsule vector in layer $l$
	\item $U_{(i,j)}^l \in \mathbb{R}$ ... $j$-th entry in $i$-th capsule vector in layer $l$.
	\item $W^l \in \mathbb{R}^{(n^l\times d^l\times n^{l+1}\times d^{l+1})}$ ... tensor holding all trans. matrices in layer $l$. 
	\item $C^{l} \in \mathbb{R}^{(n^l\times n^{l+1})}$ ... coupling coefficients from capsules $U^l$ to $U^{l+1}$
	\item $\hat{U}^l \in \mathbb{R}^{(n^l\times n^{l+1}\times d^{l+1})} $ ... vote tensor for layer $l$
\end{itemize}
However, if the context allows it, we omit specific indices to enhance readability.
Furthermore, we use the following simplified notation and abbreviations for certain variables:
\begin{itemize}
	\item $u_i \in \mathbb{R}^d$ ... $i$-th capsule vector $u_i = U_{(i,:)}$
	\item $W_{ij}^l \in \mathbb{R}^{(d^l\times d^{l+1})}$ ... trans. matrix from capsules $u_i^l$ for $u_j^{l+1}$,  $W_{ij}^l = W^l_{(i,:,j:)}$
	\item $c_{ij}^l \in \mathbb{R}$ ... coupling coefficient from capsules $u_i^l$ to $u_j^{l+1}$ $c_{ij}^l = C_{(i,j)}^l$
	\item $b_{ij}^l \in \mathbb{R}$ ... coupling coefficient prior for $c_{ij}^l$
	\item $\hat{u}^l_{j|i}\in\mathbb{R}^{d^{l+1}}$ ... vote vector from capsules $u_i^l$ to $u_j^{l+1}$ with $\hat{u}^l_{ij} = \hat{U}^l_{(i,j,:)}$
\end{itemize}

==> related_work_raw_collection.tex <==
Early work:
~\cite{cogsci/Hinton79} Reference to the hierarchy of parts.
~\cite{nips/HintonGT99} Introduction of the parse-tree.

First introduction
~\cite{icann/HintonKW11} Transforming Autoencoders

Going Public
~\cite{nips/SabourFH17} CapsNet publication.

Lots of follow-up work. In general, it is difficult to give a general statement about the state of CapsNet, as there are both technical as well as semantic developments.
There is a conceptual component to it, that makes it difficult to study!

Routing
~\cite{iclr/HintonSF18} EM Routing Expectation-Maximization Routing
~\cite{nips/AhmedT19} Star-Caps Straight Through Attentive Routing
~\cite{nips/HahnPK19} Self-Routing Capsule Networks
~\cite{aaai/RibeiroLK20} Variational Bayes Routing
~\cite{iclr/TsaiSGS20} Inverted Dot-Product Attention Routing: No Activation, So what about the parse-tree? Layer-Norm will prevent sparsity.
~\cite{nature/Mazzia21} Efficient-CapsNet: Attention Routing
~\cite{aaai/Gu21} Interpretable Graph Capsule Networks replaces the dynamic routing with a multi-head attention-based graph pooling approach

Parameter-Efficiency:
~\cite{iclr/HintonSF18} matrices instead of vectors
~\cite{cvpr/RajasegaranJJJS19} tensor instead of vectors

Advanced Features
~\cite{spl/XiangZTZX18} [Dropout] The receptive field problem was also recognized
~\cite{cvpr/RajasegaranJJJS19} [Skip connections] DeepCaps: Going Deeper With Capsule Networks skip-connections Going deeper is feasible?

More stuff
~\cite{iclr/Wang018} framed the routing in ~\cite{nips/SabourFH17} as an optimization problems.
~\cite{nips/LenssenFL18} provably equivariant capsules for MNIST.
~\cite{corr/Rawlinson2018} unsupervised learning scheme

PrimeCaps:
~\cite{nips/KosiorekSTH19} Stacked Capsule Autoencoders
~\cite{icml/SabourTYHF21} Flow Capsules: Learning PrimeCaps

Recent:
~\cite{corr/Hinton2021} GLOM was proposed

\subsubsection*{Negative results}
Depth:
~\cite{corr/XiBingJin17} First report that depth does not improve performance.
~\cite{acml/PaikKK19} The influence of depth for multiple routing algorithms. worse than simple baseline algorithms that assign the connection strengths uniformly showed that 
~\cite{prl/PeerSR21} not universal appropriators, limited in depth. No Activation, So what about the parse-tree? Layer-Norm will prevent sparsity
~\cite{corr/Rawlinson2018} Losing supervision capsules don't specialize.

Work questioning benefits:
~\cite{corr/Michels19} showed that CapsNet can be as easily fooled as ConvNets.
~\cite{cvpr/GuT20} revealed, that removing dynamic routing improves affine robustness.
~\cite{iclr/Gu2021} designed a first specific attack on CapsNets and.
~\cite{cvpr/GuT021} showed that the individual parts of the CapsNets have contradictory effects on the performance in different tasks and conclude, that with the right choice of baseline CapsNet are not more robust.

==> results_backbone_primecaps.tex <==
\begin{comment}
Was kann man sich ansehen:
- Receptive field berechnen
  - Fixiere Capsule dimension
  - Calculate number of capsules for different backbone depth and image dimensions e.g. MNIST, ImageNet.
- Activeness of prime-caps for different backbones
	- annahme: alle sind immer aktiv
	- was sein sollte: sparse caps, die fur gleich inputs mit verschiedenen poses gleich aktiviert werden und klar trennbar fur andere klassen sind.
- For image I, compare prime-caps activeness and prime-caps activeness of rotated image rot(I). Are the same primecaps active?
- %TODO: READhttps://arxiv.org/pdf/2011.13920.pdf
- Visualize which part of the input image activate a certain prime-caps
\end{comment}

\textbf{Observations}:
\begin{itemize}
	\item Usually, there is a ConvNet backbone that extracts features from an image.
	\item These features are then reshaped and constitute the first layer of Capsules, the PrimeCaps
	\item Each one of these PrimeCaps must access the full receptive field.
	\item Two options for backbone: shallow or deep ConvNet.
\end{itemize}
\textbf{Case 1}: A shallow ConvNet backbone results in:
\begin{itemize}
	\item Less abstract PrimeCaps, which is conceptually problematic due to inverse pyramid principle. Edges occur more often! 
	\item Scaling issues, as the feature maps are way too large.
	[Calculate receptive field implications for different image sizes, number of prime caps and parameters and dimension of prime caps.]. This then again results in:
	\begin{itemize}
		\item Capsule Explosion, -> Computationally expensive routing %TODO calc routing complexity
		\item Capsule deimensio explosion: Computationally expensive routing and breaks with the concept of small capsules.
	\end{itemize}
	\item a shift in the task of building more abstract and compositional objects to the routing algorithm. And as we see later, also this is limited.
	\item possibility of Sparsely activated PrimeCaps
	\item Non interpretable Capsules [show experimentally?] Show that Capsule for one sample activates for a certain part in the input and then show that it activates for another part in the transformed image.
\end{itemize}
Therefore since the approach of using shallow backbone is limited and does not scale, we can choose a deeper ConvNet backbone. \\

\textbf{Case 2}: Deeper ConvNet backbone results in:
\begin{itemize}
	\item More abstract PrimeCaps
	\item All the benefits and issues with ConvNets, especially diversification.
	\item Loss of traceability of Feature to output (really?)
	\item Still not easy to implement since pooling layers are prohibited from a conceptual perspective. Using pooling breaks with the concept.
	\item Shifts more work to the ConvNet. Hypothesis is, that all the work is done in the backbone. [Some experiments with ResNet exist and can be referenced]
	\item Experiments show, that PrimeCaps are not at all sparse, but rather dense, which breaks with the semantics. Also since all PrimeCaps are active, always, they must be routed!
\end{itemize}

\textbf{Notes on ConvNets}
\begin{itemize}
	\item ConvNets usually diversify and don`t consolidate. The diversification of the ConvNets might be shown analytically.
	\item Does the transition from place to rate coding really take place? And where?
	\item Entanglement literature does not suggest, that CNN per se learn interpretable features.
\end{itemize}

\textbf{Open questions}:
\begin{itemize}
	\item Can we show that we cannot attribute certain features to a PrimeCaps? E.g. Can we show that information about the color "red" might be scattered around many Capsules?
	\item Can we come up with a stronger theoretical claim?
\end{itemize}

\textbf{Results}:
\begin{itemize}
	\item CapsNets with shallow backbones do not scale conceptually as well as technically
	\item CapsNets with deeper backbones do not profit from routing and the PrimeCaps are dense and noisy. 
\end{itemize}
